LoRA-One: One-Step Full Gradient Could Suffice for Fine-Tuning Large Language Models, Provably and Efficiently

This paper explores how theory can guide and enhance practical algorithms, using Low-Rank Adaptation (LoRA, Hu et al. 2022) in large language models as a case study. We rigorously prove that, under gradient descent, LoRA adapters align with specific singular subspaces of the one-step full fine-tuning gradient. This result suggests that, by properly initializing the adapters using the one-step full gradient, subspace alignment can be achieved immediately and applicable to both linear and nonlinear models. Building on our theory, we propose a theory-driven algorithm, LoRA-One, where the linear convergence (as well as generalization) is built and incorporating preconditioners theoretically helps mitigate the effects of ill-conditioning. Besides, our theory reveals connections between LoRA-One and other gradient-alignment-based methods, helping to clarify misconceptions in the design of such algorithms. LoRA-One achieves significant empirical improvements over LoRA and its variants across benchmarks in natural language understanding, mathematical reasoning, and code generation. Code is available at: https://github.com/YuanheZ/LoRA-One.

==> main/linear.tex <==
\section{Analysis of LoRA under Linear Model}
\label{sec:linear}

In this section, we establish the alignment between LoRA and one gradient of full fine-tuning. This result guides us to design new strategies for speeding up practical LoRA-based algorithms, which achieve this alignment at initialization.

We formally define the negative gradient of full fine-tuning in \cref{eq:fulllinear} for the linear setting after the first step as
\begin{equation}\label{eq:G}
  {\bm G}^{\natural} := -\nabla_{\bm W} {L}(\bm W^\natural) = \frac{1}{N}\widetilde{\bm X}^{\!\top} (\widetilde{\bm Y} - \widetilde{\bm X}\bm W^\natural) \,.
\end{equation}
Note that $\widetilde{\bm X}^{\!\top}\widetilde{\bm X}$ is a non-singular square matrix \citep[Lemma 6]{zeng2023expressive}. Since left multiplication by a non-singular square matrix does not change the rank \citep[0.4.6 (b)]{horn2012matrix}, we have $\operatorname{Rank}({\bm G}^{\natural}) = \operatorname{Rank}(\Delta) = r^*$. Then, we denote the singular values of $\bm G^{\natural}$ by $\{ \lambda_i({\bm G}^{\natural}) \}_{i=1}^{r^*}$ in non-increasing order.

\subsection{Alignment under LoRA Initialization}
\label{sec:align_linear}

We first present the results for the alignment of $\bm B_t$ by recalling the notations $\bm V_{r^*}(\cdot)$ and $\bm V_{r^*,\perp}(\cdot)$.
\begin{theorem}[Alignment between ${\bm G}^{\natural}$ and $\bm B_t$]
\label{thm:alignlinearB}
    Under assumptions in \cref{sec:assumptions} for the linear setting, consider the LoRA updates \eqref{eq:ABiter} with \eqref{eq:lorainit}. We have
    \begin{align*}
        \left\|\bm V^{\!\top}_{r^*,\perp}\left({\bm G}^{\natural}\right)\bm V_{r^*}\left(\bm B_t\right)\right\|_{op} = 0\,, \quad \forall t \in \mathbb{N}_+\, .
    \end{align*}
\end{theorem}
One can see that, due to the zero initialization of $\bm B_0$ in \eqref{eq:lorainit}, after the first GD step, it holds that $\bm B_1 = \eta \bm A_0^{\!\top} \bm G^\natural$,  which has rank $\leq r^*$ and lies in the right top-$r^*$ singular subspace of $\bm G^\natural$. The subsequent GD dynamics of $\bm B_t$ is always restricted to this invariant subspace.

Next we build the alignment for $\bm A_t$ with the notations $\bm U_{r^*}(\cdot)$, $\bm U_{r^*,\perp}(\cdot)$ and $\kappa^{\natural}$ as the condition number of ${\bm G}^{\natural}$.
\begin{theorem}[Alignment between ${\bm G}^{\natural}$ and $\bm A_t$. Simplified version of \cref{thm:alignlinearA:full}]\label{thm:alignlinearA}
    For the $r \geq 2r^*$ case, under assumptions in \cref{sec:assumptions} for the linear setting, we consider the LoRA updates \eqref{eq:ABiter} with $[\bm A_0]_{ij} \sim \mathcal{N}(0, \alpha^2)$ in \eqref{eq:lorainit}.
    Then for any constant $\theta \in (0,1)$, by taking $\alpha = \mathcal{O}\Big(\theta^{\frac{3}{2}\kappa^\natural} d^{-\frac{3}{4}\kappa^\natural-\frac{1}{2}}\| {\bm G}^{\natural}\|^{\frac{1}{2}}_{op}\Big)$, 
and running gradient descent for $t^*$ steps with 
\begin{equation}\label{eq:t-aligned}
  t^* \lesssim \frac{\ln\left(\frac{\sqrt{d}}{\theta}\right)}{\ln\left(1+\eta\lambda_{r^*}\left({\bm G}^{\natural}\right)\right)} \,,
\end{equation}
we achieve the following the alignment on the left singular subspace between $\bm G^{\natural}$ and $\bm A_{t^*}$ as below
    \begin{align}\label{eq:align-t-main}
        &\left\|\bm U^{\!\top}_{r^*,\perp}( \bm G^{\natural})~\bm U_{r^*}\left(\bm A_{t^*}\right)\right\|_{op} \lesssim \theta\,,
    \end{align}
    with probability at least $1 - C_1\exp(- d) -C_2\exp(- r) -C_3\exp(- N)$ for some constants $C_1, C_2, C_3$.
\end{theorem}

{\bf Remark:} The result under the $r^* \leq r < 2r^*$ case is more complex and we defer this result to \cref{thm:alignlinearA:full}.
The choice of $\alpha$ in \cref{thm:alignlinearA} shows that  after $t^* = \Theta\left(\frac{\ln d}{\lambda_{r^*}(\bm G^{\natural})}\right)$ in \cref{eq:t-aligned}, the alignment can be achieved. Our results can cover the standard He-initialization \citep{he2015delving} if $\| \bm G^{\natural}\|_{op} \geq \Omega(d^{\frac{3}{4}\kappa^\natural})$. Requirement on $\| \bm G^{\natural}\|_{op}$ can be relaxed under smaller initialization, illustrated by \cref{fig:small-init}. \\

\begin{figure}
    \centering
    \includegraphics[width=0.999\linewidth]{pdf_figs/risk-vs-angle-corrected.pdf}
    \caption{Under \eqref{eq:lorainit}, the risk and the alignment to full one-step GD of LoRA with different $\alpha^2$ and $d$, trained via GD on task \eqref{eq:lab_linear}. \textit{Left}: the log risk under different initialization variance $\alpha^2$. The risk is defined as $\frac{1}{2}\left\|\bm A_t \bm B_t - \Delta\right\|^2_{\rm F}$. \textit{Right}: the best principal angle between the top-$r$ singular subspace of $\bm G^\natural$ and $\bm A_t$ during training. Smaller is closer. The principal angle is defined as $\min_{t}\|\bm U^{\!\top}_{r^*,\perp}( \bm G^{\natural})~\bm U_{r^*}\left(\bm A_{t}\right)\|_{op}$. More experimental details can be found in \cref{exp:toy-setting}.}
    \label{fig:small-init}\vspace{-0.2cm}
\end{figure}


The above two theorems characterize the alignment between $\bm G^{\natural}$ and $(\bm A_t, \bm B_t)$.
\cref{fig:small-init} empirically validates \cref{thm:alignlinearA} in two folds:
\textit{i}) Smaller initialization ($\alpha^2$ in the x-axis) encourages better alignment (evaluated by the principal angle), and then better generalization performance of fine-tuning (evaluated by the risk).
But in practice smaller initialization would increase the training time for convergence, as a double-edge sword.
\textit{ii)} increasing $d$ leads to longer alignment time, illustrated by \cref{eq:t-aligned}, and worse alignment performance, illustrated by the formulation of $\alpha$. 
Besides, we also verify this alignment in read-world applications by fine-tuning a T5 base model \cite{raffel2020exploring} on MRPC using LoRA, as shown in \cref{fig-angleT5}.
The mean principle angles within each layer class is computed in a similar way of \cref{fig:small-init}.
Our empirical results demonstrate that the principal angles decrease from around $1$ because of Gaussian initialization to the value around $0.2 \sim 0.4$.

{\bf Proof of Sketch:} Here we give a proof of sketch of \cref{thm:alignlinearA}.
The dynamics \eqref{eq:ABiter} can be written as 
\begin{align*}
    \underbrace{
    \begin{bmatrix}
        \bm A_{t+1} \\ \bm B_{t+1}^{\!\top}
    \end{bmatrix}
    }_{=: \bm Z_{t+1}}
    & = \underbrace{\begin{bmatrix}
        \bm I_d & \eta {\bm G}^{\natural}\\
        \eta {{\bm G}^{\natural}}^{\!\top} & \bm I_k
    \end{bmatrix} }_{=:\bm H} \underbrace{\begin{bmatrix}
        \bm A_{t} \\ \bm B_{t}^{\!\top}
    \end{bmatrix}}_{=:\bm Z_t}  +~ \mbox{nonlinear term}\,,
\end{align*}
where $\bm H$ is a time-independent matrix corresponding to the linear part of the dynamic $\bm Z^{\tt lin}_t := \bm H^t \bm Z_0$.
By Schur decomposition of $\bm H$ (see \cref{H-schur}), we can obtain the precise spectral dynamics of $\bm Z^{\tt lin}_t$ and derive the alignment between $\bm Z^{\tt lin}_t$ and ${\bm G}^{\natural}$, see \cref{psuedo-dynamics} for details.
We prove that the nonlinear term is well controlled, i.e.,
$\|\bm Z_t - \bm Z^{\tt lin}_t \|_{op} \leq \|\bm A_0\|_{op}\,, \forall t \leq t^*$, see \cref{E_t_A_0}.
Then the alignment between $\bm Z^{\tt lin}_t$ and ${\bm G}^{\natural}$ can be successfully transferred to that of $\bm Z_t$, see \cref{thm:alignlinearA:full} for details. 

We remark that previous work on matrix sensing \cite{stoger2021small,soltanolkotabi2023implicit} via a symmetrization technique cannot be directly applied to our setting. Such symmetrization technique prevents the alignment results decoupling into two factorized matrices. We extend their technique to decouple the alignment for $\bm A_t$ and $\bm B_t$ individually via Schur decomposition of $\bm H$.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\linewidth]{pdf_figs/intro_phase_transit.pdf}
    \includegraphics[width=0.48\linewidth]{pdf_figs/seed3_wo_v3.pdf}
    \caption{Comparison of the GD trajectories under \eqref{eq:spectral-init-linear} and \eqref{eq:lorainit} with two different starting points. See more experimental details in \cref{exp:toy-setting}.}
    \label{fig:phase-transi-main}
\end{figure}


\subsection{Spectral Initialization and Global Convergence}
\label{sec:linear-spectral}

\cref{thm:alignlinearA} has demonstrated the alignment on the rank-$r^*$ singular space of $\bm G^{\natural}$ and $(\bm A_t, \bm B_t)$.
In other words, if we take the SVD of $\bm G^{\natural}$ and choose the certain singular subspace for initialization in \eqref{eq:spectral-init-linear}, we can directly achieve the alignment at this initialization and recover $\Delta$ to some extent, which is the main target of this work.

By the following standard concentration result for (sub)-Gaussian data:
with probability at least $1-2C\exp(-\epsilon^2 N)$ for some constants $C>0$, we have
\begin{align}
\label{concentration-N-main}
    \left\|\widehat{\bm \Sigma} - \bm I_d\right\|_{op} \leq \epsilon:= \min\left\{\frac{1}{2\kappa}\,,\frac{c}{\kappa^3}\right\} \leq \frac{1}{2} \,.
\end{align}
Recall $\kappa$ is the condition number of $\Delta$ and $\lambda_{r^*}^*$ is the $r^*$-th singular value of $\Delta$, we have the following result at the spectral initialization.
\begin{theorem}
\label{main:linear-initial-risk}[{\color{red!80}One-step gradient can suffice}]
    Under assumptions in \cref{sec:assumptions} for the linear setting via \eqref{eq:spectral-init-linear}, taking $\epsilon$ in \cref{concentration-N-main}, then with probability at least $1-2C\exp(-\epsilon^2 N )$ for constant $C>0$, we have
    \begin{equation*}
        \| \bm A_0 \bm B_0 - \Delta \|_{op} \leq \epsilon \| \Delta \|_{op} \leq \frac{\lambda_{r^*}^*}{2} \,.
    \end{equation*}
\end{theorem}
\cref{main:linear-initial-risk} demonstrates that, after one-step full gradient, i.e., using spectral initialization \eqref{eq:spectral-init-linear}, $\bm A_0 \bm B_0$ is able to recover $\Delta$ with small error.
This is still true for nonlinear models, see \cref{A0B0-init-risk} for details.
\cref{fig:phase-transi-main} numerically validates that the starting points initialized by \eqref{eq:spectral-init-linear} are consistently closer to the set of global minimizers, whereas those initialized by \eqref{eq:lorainit} tend to be farther away across different random seeds.

Moreover, running gradient descent from points initialized by \eqref{eq:spectral-init-linear} requires significantly fewer steps to reach a global minimizer, demonstrating the advantages of \eqref{eq:spectral-init-linear}.
Due to page limit, we present the global convergence of linear models is deferred to \cref{app:lrspec} and \cref{app:precgdlr}, respectively. 
In \cref{app:lrspec}, we derive the linear convergence rate $ \left\|\bm A_{t}\bm B_{t} - \Delta\right\|_{\rm F}$.
Since the convergence will be slow if the downstream feature shift $\Delta$ is ill-conditioned, i.e., $\kappa$ is large. This motivates us to add preconditioners, then the convergence rate will be independent of $\kappa$ accordingly, see \cref{app:precgdlr} for details.
